OpenTraj: Assessing Prediction Complexity in Human Trajectories Datasets

Human Trajectory Prediction (HTP) has gained much momentum in the last years and many solutions have been proposed to solve it. Proper benchmarking being a key issue for comparing methods, this paper addresses the question of evaluating how complex is a given dataset with respect to the prediction problem. For assessing a dataset complexity, we define a series of indicators around three concepts: Trajectory predictability; Trajectory regularity; Context complexity. We compare the most common datasets used in HTP in the light of these indicators and discuss what this may imply on benchmarking of HTP algorithms. Our source code is released on Github.

==> datasets.tex <==





==> discussion_pat.tex <==

In general, most natural trajectory datasets have a local density about 0-4 p/m2 while such number is higher (2-6 p/m2) in the experimental bottleneck situation. When considering both density indicators, we can see that dataset such as wildtrack has a high global density with a low local density, which indicates the pedestrians are relatively sparse. On the contrary, low global density and high low density in Ind datasets suggests the pedestrians are more clustered. Indeed, this observation is also reflected in the interaction indicator and entropy indicator as well.

        

